Clustering Markov Decision Processes For Continual Transfer

We present algorithms to effectively represent a set of Markov decision processes (MDPs), whose optimal policies have already been learned, by a smaller source subset for lifelong, policy-reuse-based transfer learning in reinforcement learning. This is necessary when the number of previous tasks is large and the cost of measuring similarity counteracts the benefit of transfer. The source subset forms an `$\epsilon$-net' over the original set of MDPs, in the sense that for each previous MDP $M_p$, there is a source $M^s$ whose optimal policy has $<\epsilon$ regret in $M_p$. Our contributions are as follows. We present EXP-3-Transfer, a principled policy-reuse algorithm that optimally reuses a given source policy set when learning for a new MDP. We present a framework to cluster the previous MDPs to extract a source subset. The framework consists of (i) a distance $d_V$ over MDPs to measure policy-based similarity between MDPs; (ii) a cost function $g(\cdot)$ that uses $d_V$ to measure how good a particular clustering is for generating useful source tasks for EXP-3-Transfer and (iii) a provably convergent algorithm, MHAV, for finding the optimal clustering. We validate our algorithms through experiments in a surveillance domain.

==> tex_files/clustering.tex <==
\section{The Clustering Approach To Task Encoding}\label{sec_clustEnc}

\newcommand{\repm}{RM}

Recall from the Section \ref{sec_intro} that in our problem, we assume that we have a repository of MDPs and their optimal policies and we wish to use the optimal policies as the source policies for EXP-3-Transfer. Now we have the following dilemma. As the number of source policies increase, we spend more time evaluating them and accruing sub-optimal reward in the process. On the other hand, if we choose a subset of policies from the repository, then we risk leaving out policies that may have been very useful in the new task. So, essentially we are faced with the problem trading off the size and diversity of the set of source policies. 

In this section, we concretely define this tradeoff problem as optimizing a cost function, and in Section \ref{sec_findclust} we describe an algorithm to optimize this function. The cost function is defined over the set of {\em clusterings} of the repository, where each clustering corresponds to using a particular subset of policies in the repository as the source policy set. We first show how to obtain this source set given a clustering, and then define the cost function that measures how well the source set achieves the tradeoff mentioned above.

%present the basic idea of the clustering approach and derive the high level structure of a cost function for clusterings which helps us choose the best clustering for the purposes of transfer. After that, we derive two different versions of the cost function under worst-case and best-case assumptions on the target task. The worst-case cost function is pleasing theoretically, but empirically leads to poor results (please see Section \ref{sec_exp}), while for the best-case cost function the opposite turns out to be true.

\subsection{Constructing Source Policies Given Clustering}

Given the $N$ previous MDPs $\mdp_1,\mdp_2\cdots,\mdp_N$, let $\{A_1,A_2,\cdots,A_c\} \eqdef \bfA$ be a particular clustering -- that is $\cup_i A_i=$ $\{\mdp_1,\mdp_2\cdots,\mdp_N\}$ and $A_i \cap A_j = \emptyset$. The set of clusterings vary both by elements of each $A_i$, and the number of {\em cells} $A_i$.  Given a particular clustering $\bfA$, we will obtain the $c$ source policies by choosing one policy per $A_i$. To choose this policy, we define a distance function that measures how similar two MDPs are in terms of their optimal policies.

Let $\mdp_i$ and $\mdp_j$ be two MDPs with the same state and action space but different transition and reward functions. Denote by $V_i^\pi$ and $V_j^\pi$ the value of policy $\pi$ when executed, respectively, in $\mdp_i$ and $\mdp_j$ at the initial state (this can be generalized to different initial states and/or distribution over initial states very easily -- but we consider the same initial state setting to keep the presentation simple). Letting the optimal policies for the two MDPs be $\pi_i^*$, $\pi_j^*$, we define the {\em optimal policy similarity} between two MDPs as follows.
\begin{equation}\label{eq_mdpDDef}
d_V(\mdp_i,\mdp_j) \eqdef \max \{  V_i^* - V_i^{\pi_j^*}, V_j^* - V_j^{\pi^*_i} \}
\end{equation}
So this distance upper bounds how much we lose if we use the optimal policy of one MDP in the other -- in particular we have the following lemma by construction.
\begin{lemma}\label{lemma_dvOpt}
If $d_V(\mdp_i,\mdp_j) \leq \eps$, then the optimal policy of $\mdp_i$ is at least $\eps$-optimal in $\mdp_j$ and vice versa.
\end{lemma}
The definition of $d_V$ is motivated by the fact that the  goal of policy reuse is to use the optimal policy of one MDP in another. We now define the source policies given a clustering $\bfA$:
\begin{definition}\label{def_srcPol}
Given a clustering $\bfA = \{A_1,A_2,\cdots,A_c\}$ the source policy corresponding to a cluster $A_i$ is the optimal policy $\rho_i$ of $\mdp^i$, where:
\begin{equation}\label{eq_landmark_dV}
\mdp^i \eqdef \argmin_{\mdp \in A_i} \max_{\mdp' \in A_i} d_V(\mdp,\mdp')
\end{equation}
(ties broken in terms of order in the sequence $\mdp_1,\mdp_2,\cdots,\mdp_N$).
\end{definition}
The definition is illustrated in Figure \ref{fig_clustIll} and it means the following.  $\mdp^i$ is the element of $A_i$ that minimizes the maximum $d_V$ distance to the other elements of the cluster, and hence, by Lemma \ref{lemma_dvOpt}, is in a worst case sense the best representative of the MDPs in cluster $A_i$. Given our strategy of choosing the source policies given clusterings, we now discuss how to evaluate such clusterings.



\begin{figure}[h]
\begin{center}
\includegraphics[scale=0.5]{clust_illustrate.pdf}
\end{center}
\caption{This figure sketches our basic approach to deriving the source policies. The black circles represent our set of previous $N$ MDPs. The goal is to them into $c$ clusters and then derive $c$ source policies from the $c$ source tasks. The figure illustrates the idea for $c = 3$. Each cluster is an analogue of an  $\eps$-ball in a metric space according to $d_V$ (\ref{eq_mdpDDef}). The source MDPs form an analogue  of an $\eps$-net  over the set of previous MDPs with respect to $d_V$. The function $d_V$ measures how well the policy of one MDP performs in the other -- and hence the source policies being an $\eps$-net implies that, given any MDP in the set of previous MDPs, there is at least one source policy which has performance that is `$\eps$-close' to the performance of the optimal policy of the previous MDP. }\label{fig_clustIll}
\end{figure}


\subsection{Cost Function of a Clustering}\label{sec_mdpN1prev}

Let $\bfA = \{A_1,A_2,\cdots,A_c\}$ be a clustering with the $c$ source policies $\rho_1,\rho_2,\cdots,\rho_c$ chosen as defined in the previous subsection. Our goal in this section will be to quantify the regret of EXP-3-Transfer with respect to any $\pi^*_k$ when executed on the new task $\mdp_{N+1}$ for $T$ episodes, where $\pi^*_k$ is the optimal of $\mdp_k$ in the repository $\{\mdp_1,\mdp_2,\cdots,\mdp_N\}$. We will consider the case where EXP-3-Transfer is run with arms $\rho_1,\rho_2,\cdots,\rho_c$, and hence this regret will quantify how good the clustering $\bfA$ is for transfer -- in particular, the lower the regret, the more preferable the clustering. As a result, the regret will serve as the cost function for choosing a clustering to derive the source policies. Before proceeding, note that in Theorem \ref{thm_EXPBound}, we computed the regret between EXP-3-Transfer and $\rho_i$ -- in this section we extend those results to derive the regret with respect to $\pi^*_k$.

%Our goal in this section will be to quantify the difference in the expected accumulated discounted reward between  EXP-3-Transfer and the best policy hindsight in the set $\{\pi_i^*\}_i \cup \{\mbox{Q-learning policy}\}$. We quantify the difference for the case when the policies are used on the new MDP $\mdp_{N+1}$ for $T$ episodes, where EXP-3-Transfer using the arms $\rho_i$ and Q-learning, to the expected accumulated reward of the policy that obtains best 

To begin, let the diameter of a cluster $A_i$, and the mean diameter of the clustering $\bfA$  be:
\begin{equation}\label{eq_bareps}
\eps_i \eqdef  \max_{\mdp \in A_i} d_V(\mdp^i, \mdp), \;\;\; \bar{\eps} \eqdef \frac{1}{N} \sum_{i=1}^c |A_i|\eps_i
\end{equation}
So $\bar{\eps}$ is the average diameter of the clusters, weighted by the size of the clusters. Therefore, $\bar{\eps}$ gives the average distance from a cluster center $\mdp^i$ to an element of the cluster. As such, $\bar{\eps}$ measures how much of the diversity in the repository is captured by the chosen clusters.  The smaller $\bar{\eps}$, the smaller the average $d_V$ distance between the cluster centers $\rho^i$ and the MDPs in $A_i$, and hence more of the diversity of policies in the repository is captured by the $\rho^i$. 

\footnotetext[2]{A worst case quantification is also possible. However, the assumptions underlying the worst case seems too weak, and the cost function correspondingly not sufficiently discriminating -- i.e. it identifies MDPs that are intuitively dissimilar as being similar. In particular in our experiments, we found this cost function to not give us the intuitive clusters. We discuss this function further in appendix \ref{app_worstCase}.}


Using these, we can give an average case quantification\footnotemark of the performance of a clustering $\bfA$ when used to generate the source policies and used in EXP-3-Transfer. Let the new MDP $\mdp_{N+1}$ have transition and reward functions $R_{N+1}$ and $P_{N+1}$. Let $\forall s,a$ $|R_k(s,a) - R_{N+1}(s,a)| \leq K_k$ and $|P_k(.|s,a) - P_{N+1}(.|s,a)|  \leq K'_k$ where $R_k$ and $P_k$ are the reward and transition functions for MDP $\mdp_k$. Additionally let
\begin{equation}\label{eq_Kidef}
K(k) \eqdef \frac{K_k + \gamma K'_k R_{max}}{(1-\gamma)^2}, \mbox{ and } \;\;\; \bar{K} \eqdef \frac{1}{N}\sum_i K(k) 
\end{equation}
$K(k)$ measures how far each $\mdp_k$ is from the new MDP $\mdp_{N+1}$  in terms of the reward and transition function. We have the following result which derives from Theorem \ref{thm_EXPBound}.
\begin{lemma}\label{lemma_avgQuant}
If EXP-3-Transfer is run with source policies derived from $\bfA$ using definition \ref{def_srcPol} with $\beta$ set as in Theorem \ref{thm_EXPBound},
then for $\pi^*_k \in A_i$, such that EXP-3-Transfer did not eliminate $\rho_i$ by step $T$, the following is true: 
\begin{equation}\label{eq_avgQuant1}
V^{\pi^*_k}_{N+1} - \expc_{R,P}\left [\expc_{E3T}\left [ \sum_{t=1}^T \bar{x}_{i_t}(t) \bigg |\rho_i \in C_T \right] \right ] \leq g(c) + \eps_i + 2K(k)
\end{equation}
Additionally, with probability $1-\delta$, with respect to randomization due to the target MDP $\mdp_{N+1}$, for each $\pi^*_k \in A_i$ such that $\rho_i$ was eliminated, there exist $\rho_{i'}$ such that 
\begin{equation}\nonumber
V_{N+1}^{\pi^*_k} \leq V_{N+1}^{\rho_{i'}} + \eps_i + 2K(k)
\end{equation}
\end{lemma}
The proof is in Appendix \ref{app_proofs}. Now recall that we assume that each MDP $\mdp_k$ in the repository is equally likely to be the one with the minimum $K(k)$. Furthermore, if we consider the bounding case of when $\delta = 1$, none of the policies $\rho_i$ are eliminated and in this case the bound (\ref{eq_avgQuant1}) applies to all the MDPs in the repository. By taking the average of (\ref{eq_avgQuant1}) over all the MDPs, we get the upper bound of the average regret all the MDPs in the repository:
\begin{equation}\label{eq_avgQuant}
g(c) + \bar{\eps}  + 2\bar{K}
\end{equation}
We now define our cost function in the following way. $K(k)$ defined above depends on the repository of $\mdp_k$s which we do not control or make any assumptions about. Hence, we associate with each cluster $\bfA$ the parameters $(c,\bar{\eps})$, defined at the beginning of this section, and use (\ref{eq_avgQuant}) to define the following cost:
\begin{definition}\label{def_cost2}
The cost of a clustering $\bfA$ with parameters $(c,\bar{\eps})$ is defined to be:
\begin{equation}
cost(\bfA) \eqdef g(c) + \bar{\eps}
\end{equation}
\qed
\end{definition}

%However, $\bar{K}$ is a property of the $\mdp_i$s, which we do not make any assumptions about. Hence, we can ignore $\bar{K}$ and use $g(c) + \bar{\eps}$ as an average case quantification of the performance of cluster $\bfA$. 





\subsection{Hardness of finding the Optimal Clustering}\label{sec_clustHard}

In this section we introduce the problem of finding the clustering that minimizes $cost()$. We argue that optimizing the cost function is hard, which sets the stage for developing our discrete optimization algorithm in the next section. Specifically we will show that it is hard to optimize an upper bound $cost_{m}()$ of $cost()$ where $cost()$ was defined in Definition \ref{def_cost2}. To that end, define the average max-diameter of a clustering $\bfA$ to be:
\begin{equation}\label{eq_avgMaxdiam}
\bar{\eps}_m = \frac{1}{N}\sum_i |A_i| \bar{\eps}_m^i, \mbox{ where } \eps_m^i = \frac{1}{|A_i|} \sum_{\mdp \in A_i} \max_{\mdp' \in A_i} d_V(\mdp,\mdp')
\end{equation}
Now define, 
\begin{definition}
Define $cost_{m}(\bfA) \eqdef g(c)+ \bar{\eps}_m$.
\end{definition}
We have the following relationships.
\begin{lemma}
The parameter $\bar{\eps}_m$ of $\bfA$ is an upper bound on the parameter $\bar{\eps}$ of $\bfA$ defined in (\ref{eq_bareps}). Furthermore, $cost_{m}$ upper bounds $cost$.
\end{lemma}
\begin{proof}
This follows directly from the definition of $\bar{\eps}$ -- in particular, 
$\bar{\eps}_m$ upper bounds $\bar{\eps}$  because $\max_{\mdp,\mdp' \in A_i}  d_V(\mdp,\mdp')$ $> \min_\mdp \max_{\mdp'}d_V(\mdp,\mdp')$ $= d_V(\mdp^i,\mdp)$. The second part of the lemma now follows by the definitions of  $cost()$ and $cost_m()$.
\end{proof}

We reduce the minimum clique-cover problem \citep{karp:1972} to the problem of finding the clustering that minimize  $cost_{m}$ and hence establish that it is NP-complete. We start by describing the clique cover problem. Let $G  = (V,E)$ be a graph where $V$ is the set of vertices and $E$ is the set of edges. A subset $V' \subset V$ is a clique if for any $v,v' \in V$, there is an edge $(v,v') \in E$. The minimum clique cover problem is finding a partition $V_1,V_2,\cdots,V_n$ of $V$ such that each $V_i$ is a clique and $n$ is minimum -- that is there exists no other partition with $V'_1,V'_2,\cdots,V'_m$ of $V$ such that each $V'_i$ is a clique and $m < n$. We have the following theorem for $cost$.
\begin{theorem}\label{thm_npcomplete}
Given a graph $G = (V,E)$, in time polynomial in the $|V|$ and $|E|$, we can reduce the minimum clique cover problem for $G$ to finding the clustering $\bfA^*$ of MDPs $\mdp_1,\mdp_2,\cdots,\mdp_{|V|}$, with all $\mdp_i$ defined on the same state and action spaces, where $\bfA^* \eqdef \argmin_{\bfA \in\clstngs} cost_{m}(\bfA)$.
\end{theorem}
The proof is given in Appendix \ref{app_proofs}. Since the clique cover problem is NP-complete, we immediately have the following corollary. 
\begin{corollary}
Finding the clustering minimizing the upper bound $cost_{m}()$ of $cost()$ is NP-complete. 
\end{corollary}
Unfortunately, we do not yet have a proof that minimizing $cost()$ is hard -- but the fact that minimizing the upper bound $cost_m()$ is hard, leads us to conjecture that minimizing $cost()$ is hard as well. For this reason, to optimize the $cost()$ function we need a discrete optimization function, which we will develop in the next section.

We end this section by contrasting our approach to previous approaches to clustering MDPs in TLRL (for instance \citep{wilson_fern_ray_tadepalli:2007}). In prior work, MDPs are typically characterized by a finite number of real valued parameters, and the distance between parameters determine how similar the MDPs are. These MDPs can then be clustered by, for instance, putting the non-parametric Dirichlet process prior over the parameters, and then using Monte Carlo inference methods to find the clustering that maximizes the posterior probability. 

Since our similarly between MDPs is based on policies, to apply this approach to our case, we need (1) a relatively compact parametric representation of optimal policies, and (2) a metric that relates the policy-parameters to values of policies and (3) that optimal policies uniquely characterize MDPs. (1) seems difficult for interesting policies, and (2) seems reasonable only for `linear' domains -- i.e. domains where a small change in policy results in a corresponding small change in its value. (3) runs completely counter to one of our main motivations for using policy based clustering, which is that different MDPs might have identical or  near-identical optimal policies. So given all these, we were motivated to construct a clustering algorithm adapted to our policy based clustering of MDPS. We also compare our method and the method of \cite{wilson_fern_ray_tadepalli:2007} in Section \ref{sec_colGrid}, where in a simplified version of their domain, our approach recovers better clusterings.



% it is typically not possible to characterize interesting policies using a relatively small number of parameters and more importantly (2) optimal policies do not uniquely characterize MDPs and (3) . We discuss the differences between our approach and these previous approaches in more detail in Section \ref{sec_colGrid}.


%It is worth discussing at this point the fact that in prior work on transfer learning where clustering was used [citation], people used a Bayesian approach to clustering. In that case, MDPs are defined to be similar if the distributions defining them are the same. In that case, one can put a non-parametric prior on the space of distributions that's generating the MDP transition and reward distribution, and then use a Bayesian non-parametric approach to clustering the MDPs. This approach is difficult to apply in our case where we define MDPs to be similar in terms of their optimal policy. There is not a natural way to describe a generative process for MDPs in terms of their optimal policies, because the optimal policy does not uniquely identify an MDP. Hence, we need a more novel approach, which is described in the next section.



%\clearpage
%
%and then choose optimal policies of the representative element of the $A_i$s as the $c$ source policies. We will set the representative element $\mdp^i$ of $A_i$ to be the MDP whose optimal policy $\rho_i$ does as well as possible in the a-priori unknown $\mdp_{N+1}$ as the optimal policy of any other elements $A_i$. The problem now is to find the best possible clustering $\bfA$ and for that we need an objective or cost function for the clustering $\bfA$ when it is used to learn the unknown $\mdp_{N+1}$ using EXP-3-Transfer. We may define it as follows:
%
%
%Our goal is to, given $N$ previous MDPs, choose a subset $c$ of those MDPs whose optimal policies will be used as input to EXP-3-Transfer as the $c$ source policies when solving the $N+1^{th}$ MDP $\mdp_{N+1}$. Here, the number $c$ as well as the MDPs themselves are to be determined by our learning algorithm. To that end, we begin by noting that  the regret bound of EXP-3-Transfer in Corollary \ref{corollary_EXPBound} increases monotonically with the number of source policies. This indicates that we should have as few source policies as possible. However, at the same time, if we have fewer source policies, we risk leaving out a previous optimal policy $\pi_k^*$ of a previous MDP $\mdp_k$ that may have obtained high discounted return in $\mdp_{N+1}$. Hence, in choosing the source policies, we need to achieve a tradeoff between (a) additional regret suffered by having too many arms, and the (b) additional regret incurred by not having a 'good' MDP in the subset of $c$ MDPs. In particular, we need a cost function that quantifies the value of a subset c in terms of these two additional regrets.
%
%Since, we are using EXP-3-Transfer for transfer learning, regret (a) is obtained from the bound in Theorem \ref{thm_EXPBound}. However, we need some additional work to get (b), and by summing them together, we will have our cost function. To derive (b), we will proceed  as follows. Since 
%
%
%In order to quantify this tradeoff, we need to 
%
%
%
%Our approach to choosing the source policies will be as follows (illustrated in  \ref{fig_clustIll}). We will divide the $N$ previous MDPs into $c$ different groups or clusters $\{A_1,A_2,\cdots,A_c\} \eqdef \bfA$ and then choose optimal policies of the representative element of the $A_i$s as the $c$ source policies. We will set the representative element $\mdp^i$ of $A_i$ to be the MDP whose optimal policy $\rho_i$ does as well as possible in the a-priori unknown $\mdp_{N+1}$ as the optimal policy of any other elements $A_i$. The problem now is to find the best possible clustering $\bfA$ and for that we need an objective or cost function for the clustering $\bfA$ when it is used to learn the unknown $\mdp_{N+1}$ using EXP-3-Transfer. We may define it as follows:
%\begin{multline}\label{eq_comp}
%\mbox{ regret of EXP-3-Transfer w.r.t. one of the $c$ source policies $\rho_i$} \\
% + \mbox{ minimum regret of using $\pi^*_k$ in the unknown $\mdp_{N+1}$}\\
%+ \mbox{ maximum over regret of a $\rho_i$ w.r.t. an MDP $\mdp_k \in A_i$}\
%\end{multline}
% The first component in (\ref{eq_comp}) is the bound in Corollary \ref{corollary_EXPBound}. In Sections \ref{sec_mdpN1arb}  and \ref{sec_mdpN1prev} we derive two different ways to get the second and third component (recall from Section \ref{sec_prelim} that the regret of a policy $\pi$ is $V^*_k(s^\circ) - V^\pi_k(s^\circ)$ where $s^\circ$ is the initial state).  Both approaches build on the policy based distance between MDPs that we introduce in Section \ref{sec_polDist}. But then they diverge in terms of the assumptions made on $\mdp_{N+1}$. The first cost function assumes that the $\mdp_{N+1}$ is arbitrary, while the second one assumes that $\mdp_{N+1}$ is one of the $N$ previous MDPs. Correspondingly, we refer to these as, respectively, the worst case and best case assumption on $\mdp_{N+1}$.
%

%
%
%\subsection{A Policy Based Distance Between MDPs}\label{sec_polDist}
%
%In this section we define a distance between MDPs based on their optimal policies.  Therefore  $\min_i \max_{\mdp \in A_i} d_V(\mdp^i,\mdp)$ gives us the second term of (\ref{eq_comp}). For the third term we need to bound the $d_V$ distance between any arbitrary $\mdp^i$ and $\mdp_{N+1}$ as a function of the $d_V$ distance between a $\mdp^i$, $\mdp \in A_i$ and $\mdp$, $\mdp_{N+1}$. This is possible if either $d_V$ is a metric or if $\mdp_{N+1}$ has optimal policy identical to another previous MDP. Since in the first case we need to make no assumptions about $\mdp_{N+1}$, this corresponds to a `worst case' assumption, while the second case corresponds to a `best case' assumption. However, the worst case is not directly achievable because $d_V$ is not a metric (the proof is in appendix \ref{app_proofs}):
%\begin{lemma}\label{lemma_dvnometric}
%There exists $\mdp_1,\mdp_2,\mdp_3$ all defined on the same state and action space such that the function $d_V$ does not satisfy the triangle inequality: $d_V(\mdp_1,\mdp_3) \geq d_V(\mdp_1,\mdp_2) + d_V(\mdp_2,\mdp_3)$. Hence $d_V$ is not a metric in general.
%\end{lemma}
%So, in Section \ref{sec_mdpN1arb} we develop a Lipschitz metric that `envelops' $d_V$, and develop a cost function under the worst-case assumption. In Section \ref{sec_mdpN1prev} we develop the cost function under the best case assumption. 
%
%
%%In this section we show how to cluster a set of $N$ previous MDPs into $c$ clusters to derive $c$ source tasks for input to EXP-3-Transfer. To that end, we first derive present a cost-function for clusterings, which gives us a discrete optimization problem. To solve this, we present simulated annealing with stochastic temperature changes, a novel, provably convergent, version of simulated annealing.  In the sequel we assume a fixed VPL metric $d$ and a set of previous MDPs $\mdp_1,\mdp_2,\cdots,\mdp_N$. 


==> tex_files/wilson.tex <==
In~\cite{wilson}, the unknown distribution of tasks in a multi-task reinforcement learning problem is modelled using a hierarchical infinite mixture model. The two-layer model allows capturing a previously-unknown number of classes of MDPs as well as finding the distribution of parameters in each class. For any new task, the model helps as a prior in the  parameter space allowing a faster initial solution to be generated, which learning would afterwards optimise.

To compare this approach with ours, we consider a simplified version of the  coloured maze domain of~\cite{wilson}, where each square of a grid world is coloured with one of two possible colours. The agent's task is to optimise rewards when navigating from one corner to the opposite corner using the 4 canonical movements. With deterministic transitions, the variability in the tasks comes from the reward weights of the two colours of the domain. The agent is rewarded the sum of the   colour weights of the current cell and the adjacent four. We assume that weights $w\in[0,1]$. Thus, each task is completely identified by a 2D parameter in the unit square. This is intended to make it simpler to present the resulting clusterings.

We sample 50 tasks randomly from the unit square and pass them to both the hierarchical infinite mixture model and to our framework. Figure~\ref{fig:col_wilson_clus} shows the clustering of~\cite{wilson}. Figure~\ref{fig:col_our_clus} shows the clustering of our method. Note that all the tasks that lie on the same line that goes through the origin are equivalent as they have the same colour weight ratio, and thus have the same optimal policy with scaled values. For that, we expect our method to be able to capture this fact and summarise the set of MDPs into a small set of landmark MDPs. On the other hand, modelling the tasks based on  task parameters will fail to realise that fact and end up having many clusters with very similar policies because they share a parameter local neighbourhood.



\begin{figure}[h!]
 \centering 
\subfloat[Clustering of~\cite{wilson}]{
    \includegraphics[width=30mm;height=30mm;]{colour_wilson_clus}
    \label{fig:col_wilson_clus}
}
\subfloat[Clustering of our framework]{
      \includegraphics[width=30mm;height=30mm;]{colour_our_clus}
\label{fig:col_our_clus}
}
}

\caption{The tasks in parameters space of the coloured maze domain. Each dot is a one of the sampled tasks. The first plot shows clustering using a hierarchical infinite mixture model. The asterisks are the means of recovered clusters and the circles are three standard deviations. The second plot shows clustering with our framework. Each colour represents a separate class. Note how our method captures the similarity in policy much more closely than methods that cluster in parameter space.}

\end{figure}

